RepCNN: Micro-sized, Mighty Models for Wakeword Detection

Always-on machine learning models require a very low memory and compute footprint. Their restricted parameter count limits the model's capacity to learn, and the effectiveness of the usual training algorithms to find the best parameters. Here we show that a small convolutional model can be better trained by first refactoring its computation into a larger redundant multi-branched architecture. Then, for inference, we algebraically re-parameterize the trained model into the single-branched form with fewer parameters for a lower memory footprint and compute cost. Using this technique, we show that our always-on wake-word detector model, RepCNN, provides a good trade-off between latency and accuracy during inference. RepCNN re-parameterized models are 43% more accurate than a uni-branch convolutional model while having the same runtime. RepCNN also meets the accuracy of complex architectures like BC-ResNet, while having 2x lesser peak memory usage and 10x faster runtime.

==> rebuttal.tex <==
\section{Rebuttal}

Thanks to all the reviewers for their valuable feedback. We would like to address the main takeaways from the feedback as follows:

Novelty:

The main novelty of our paper is proving that in constrained parameter space re-parameterized models are beneficial both in terms of memory and latency, while meeting the performance of complex architectures. Prior works have shown these experiments on much larger scale models while our experiments are restricted to tiny models where one might believe number of parameters or complexity of the models would dictate the accuracy. We have shown that re-parameterizable models strike a good balance with low memory costs while performing equally well as complex models. In addition, memory constrained models do not consider the total runtime cost of a model, i.e. parameters + activations during execution. Complex models like BC-ResNet have a trade-off for number of model parameters with runtime memory cost. We have shown that re-parameterizable models are more memory efficient. 

To further justify our claims we verified our model on Google Speech Commands as well. We have found that a RepCNN model with 10k parameters consumes only 1.2 MB to run with 0.7ms latency while achieving > 96.5\% accuracy. A BCResNet model designed to get such accuracy needs 30k parameters leading to a total memory cost of 1.7MB with 2ms runtime latency.

Additionally, the proposed architecture is different from the ones used in vision applications because here the model operates in fully causal mode.
%In other words complex neural architectures for constrained parameters spaces can be replaced with such re-parameterizable models for wake-word detection. 

% Developing models with very few parameters is difficult because of the limited amount of information that can be stored within such strict limits. However, memory constrained models do not consider the total runtime cost of a model, i.e. parameters + activations during execution. Complex models like BC-ResNet have a trade-off for number of model parameters with runtime memory cost. In this paper we have shown that simpler neural network graphs can meet the performance of complicated graphs while being far more efficient overall. To further justify our claims we verified our model on Google Speech Commands as well. We have found that a RepCNN model with 10k parameters consumes only 1.2 MB to run with 0.7ms latency while achieving > 96.5\% accuracy. A BCResNet model designed to get such accuracy needs 30k parameters leading to a total memory cost of 1.7MB with 2ms runtime latency.

% Additionally, the proposed architecture is different from the ones used in vision applications because here the model operates in fully causal mode.

Operating Point Selection:

The operating point was selected to show that the RepCNN model is able to match the performance of complex architecture models like BCResNet, and from the DET curve shared in the paper it is evident that lowering FA/hr from that point our model is able to consistently do better in FRR compared to the other models. Such tiny models often are operated at high FA/hr for high recall with reasonable precision followed by a big parameter model for more precise detection in a cascaded system for wake-word detection. 

Loss curves for BC-ResNet:

Thanks to Reviewer #5 for pointing it out. We will add it to the paper.

Future Work:

We were not able to explore other architectures using such re-parameterization because the motivation behind this work was to make it compute and memory efficient. Additional complexity in the neural network graph has implied latency or memory costs during runtime.






The main novelty of our paper lies in proving that in a constrained parameter space, re-parameterized models offer benefits in terms of both memory and latency, while maintaining the performance of complex architectures. Previous studies have conducted similar experiments on much larger scale models. However, our experiments are limited to tiny models where one might expect the number of parameters or the complexity of the models to determine accuracy. We demonstrate that re-parameterizable models strike a good balance with low memory costs while performing equally well as complex models. Moreover, memory-constrained models typically do not consider the total runtime cost of a model, i.e., parameters + activations during execution. Complex models like BC-ResNet involve a trade-off between the number of model parameters and runtime memory cost. We show that re-parameterizable models are more memory-efficient.

To further support our claims, we verify our model on Google Speech Commands as well. We find that a RepCNN model with 100k parameters consumes only 1.2 MB to run with a latency of 0.7ms while achieving >96.5\% accuracy. In comparison, a BCResNet model designed to achieve such accuracy needs 30k parameters, resulting in a total memory cost of 1.7MB with a 2ms runtime latency.

Additionally, the proposed architecture differs from those used in vision applications because the model operates in fully causal mode.
